Representation Bayesian Risk Decompositions and Multi-Source Domain Adaptation

We consider representation learning (hypothesis class $\mathcal{H} = \mathcal{F}\circ\mathcal{G}$) where training and test distributions can be different. Recent studies provide hints and failure examples for domain invariant representation learning, a common approach for this problem, but the explanations provided are somewhat different and do not provide a unified picture. In this paper, we provide new decompositions of risk which give finer-grained explanations and clarify potential generalization issues. For Single-Source Domain Adaptation, we give an exact decomposition (an equality) of the target risk, via a natural hybrid argument, as sum of three factors: (1) source risk, (2) representation conditional label divergence, and (3) representation covariate shift. We derive a similar decomposition for the Multi-Source case. These decompositions reveal factors (2) and (3) as the precise reasons for failure to generalize. For example, we demonstrate that domain adversarial neural networks (DANN) attempt to regularize for (3) but miss (2), while a recent technique Invariant Risk Minimization (IRM) attempts to account for (2) but does not consider (3). We also verify our observations experimentally.

==> Makefile <==
### Makefile --- 

TARGETS = paper

%: %.tex
	latexmk -g -pdf -silent $@ # generate pdf
	latexmk -c $@ # clean up regeneratable files
	rm -f *.bbl

all: pdf

pdf: ${TARGETS}

clean:
	@echo cleaning up...
	rm -f *.bbl *.fdb_latexmk *.ps *.dvi *.aux *.bbl *.blg *.brf *.cb *.cb2 \
		 *.idx *.ilg *.ind *.inx *.log *.mpx *.toc *.out *.pstex_t \
		 *.fig.bak  *.ps_e *~ *.tex.* *.thm *.fls



==> conclusions.tex <==
We presented fine-grained risk decompositions for domain adaptation in the
representation learning setting. It allows us to identify the conditions for
successful invariant representation learning. In particular, we use them to
investigate several interesting failure examples of existing approaches such as
DANN and IRM, revealing that the regularizations in these approaches are
complementary. Our risk bounds show that explicitly incorporating representations
can provide novel implications, and open an avenue for designing future algorithms
for representation learning in domain adaptation. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

